On Learning the Structure of Clusters in Graphs

Graph clustering is a fundamental problem in unsupervised learning, with numerous applications in computer science and in analysing real-world data. In many real-world applications, we find that the clusters have a significant high-level structure. This is often overlooked in the design and analysis of graph clustering algorithms which make strong simplifying assumptions about the structure of the graph. This thesis addresses the natural question of whether the structure of clusters can be learned efficiently and describes four new algorithmic results for learning such structure in graphs and hypergraphs. All of the presented theoretical results are extensively evaluated on both synthetic and real-word datasets of different domains, including image classification and segmentation, migration networks, co-authorship networks, and natural language processing. These experimental results demonstrate that the newly developed algorithms are practical, effective, and immediately applicable for learning the structure of clusters in real-world data.

==> chapters/conclusions.tex <==
\chapter{Conclusion} \label{chap:conclusion}
In this thesis, we have seen several new algorithms for learning the structure of clusters in graphs and hypergraphs.
Along the way, we have touched on many different approaches and techniques for graph clustering including classical spectral clustering, local clustering, and hypergraph diffusion methods.
It is clear that by taking the structure of clusters into account, it is possible to develop significantly improved methods for graph clustering and to analyse complex datasets which appear in many real-world applications.
The techniques introduced in this thesis also raise many open questions and directions for future work, ranging from theoretical questions to details of practical applications.

In Chapters~\ref{chap:tight}~and~\ref{chap:meta} we studied the spectral clustering algorithm and found that when the clusters possess a clear high-level structure, using fewer than $k$ eigenvectors in order to find $k$ clusters performs better than using $k$ eigenvectors.
This result has immediate practical applications, including an extremely effective and simple algorithm for image segmentation with spectral clustering.
Despite its long history, there is still much to learn about the spectral clustering algorithm, such as how to determine the optimal number of eigenvectors to use.
The image segmentation algorithm would also benefit from further study.
In particular, the optimal method for constructing a similarity matrix from an image remains unclear.

In Chapter~\ref{chap:local}, we saw that densely connected clusters in graphs can be learned locally using random walks on the graph's double cover.
This raises an interesting question of whether other cluster structures can also be learned locally, or indeed whether there is a general method for finding clusters with arbitrary structures.
Another direction is to consider the problem of finding clusters in signed graphs.
One can view the edges in the interstate dispute graph, for example, as representing \emph{negative} relationships between vertices and so it would be insightful to study similar problems in graphs containing both positive and negative edges.
Such an algorithm could be used to find opposing groups on social media platforms, for example, and could help us to understand whether social media encourages groups with differing views to become more polarised over time.

Finally, in Chapter~\ref{chap:hyper} we introduced a new spectral hypergraph operator which generalises the signless graph Laplacian, and saw how this operator can be used to learn densely connected clusters in hypergraphs.
The field of spectral hypergraph theory is still in its infancy and many questions remain.
A significant challenge in this area is the non-linearity of the hypergraph Laplacian and signless Laplacian operators, which
makes the study of their spectrum particularly difficult.
However, as established in the examples in Chapter~\ref{sec:numeigs}, these operators can have many eigenvectors and further studying their spectrum is likely to offer new insights.
For example, it may be possible to develop a spectral clustering algorithm for hypergraphs based on the eigenvectors of the non-linear hypergraph Laplacian operator.

The results presented in this thesis have all been supported by extensive evaluation on real-world data, indicating their immediate applicability.
It is crucial that future research in spectral graph and hypergraph theory continues to have this grounding in application.
Furthermore, there is a need for more accessible and reliable implementations of effective algorithms for data analysis.
Future research should prioritise such implementations in order to support further research as well as to bridge the gap between theory and practice.
